Cross-lingual hate speech detection based on multilingual domain-specific word embeddings

Automatic hate speech detection in online social networks is an important open problem in Natural Language Processing (NLP). Hate speech is a multidimensional issue, strongly dependant on language and cultural factors. Despite its relevance, research on this topic has been almost exclusively devoted to English. Most supervised learning resources, such as labeled datasets and NLP tools, have been created for this same language. Considering that a large portion of users worldwide speak in languages other than English, there is an important need for creating efficient approaches for multilingual hate speech detection. In this work we propose to address the problem of multilingual hate speech detection from the perspective of transfer learning. Our goal is to determine if knowledge from one particular language can be used to classify other language, and to determine effective ways to achieve this. We propose a hate specific data representation and evaluate its effectiveness against general-purpose universal representations most of which, unlike our proposed model, have been trained on massive amounts of data. We focus on a cross-lingual setting, in which one needs to classify hate speech in one language without having access to any labeled data for that language. We show that the use of our simple yet specific multilingual hate representations improves classification results. We explain this with a qualitative analysis showing that our specific representation is able to capture some common patterns in how hate speech presents itself in different languages. Our proposal constitutes, to the best of our knowledge, the first attempt for constructing multilingual specific-task representations. Despite its simplicity, our model outperformed the previous approaches for most of the experimental setups. Our findings can orient future solutions toward the use of domain-specific representations.

==> Acc.tex <==
\begin{table}[]
\caption{Word translation $Accuraccy_{10}$}
\begin{tabular}{c | c  c c}
\hline
 Model & EN\_ES & EN\_IT & ES\_IT \\ \hline
 Hate     & 54.67&  48.93 & 49.8     \\ \hline
 Muse     & 61.32&  64.32 & 51.54 \\ \hline
\end{tabular}
\end{table}

==> Cualitative_evaluation.tex <==
\begin{table*}
\caption{Equivalent terms in different languages using equation \ref{eq1}.}
\label{tab:Cualitative_evaluation}

\begin{tabular}{ c c c c c c c }

 & \multicolumn{2}{c}{\Small{Nearest Neighbor in Vector Space}} & \multicolumn{2}{c}{\Small{Nearest Neighbors Term in Hateful Data}}  & \multicolumn{2}{c}{\Small{Nearest Neighbour Term in No-Hateful Data}} \\ 

\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%

 \Small{English Seed Term} & \Small{Spanish}  & \Small{Italian}  & \Small{Spanish} & \Small{Italian} & \Small{Spanish} & \Small{Italian}\\

\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}

 % \parbox{7em}{\centering\Tiny}               
\Small{muslims} &\Small{musulmanes}   &   \Small{musulmani}  & \parbox{7em}{\centering\Tiny escoria, 0.63,\\  fascistas, 0.62,\\ fascista, 0.61}   & \parbox{7em}{\centering\Tiny fare, 0.66,\\ islamico, 0.66,\\ terroristi, 0.65} & \parbox{7em}{\centering\Tiny cultural, 0.60,\\ retweeted, 0.60,\\ libre, 0.60)}   & \parbox{7em}{\centering\Tiny ancora, 0.67,\\ fare, 0.66, \\islamico, 0.66} \\ 

%\cmidrule(lr){2-8}
% \Small{nicca} &  \parbox{7em}{\centering\Tiny }    & \parbox{7em}{\centering\Tiny }   & \parbox{7em}{\centering\Tiny  mongolo, 0.58,\\ tipo, 0.58,\\ gordo, 0.57}   & \parbox{7em}{\centering\Tiny merda, 0.56,\\ vogliono, 0.56,\\ islam , 0.56} &  \parbox{7em}{\centering\Tiny }  &\parbox{7em}{\centering\Tiny }   \\
% \cmidrule(lr){2-7}
\Small{retarded} & \Small{imbecil}
    &  \Small{idiota}  & \parbox{7em}{\centering\Tiny gilipollas, 0.59,\\ cara, 0.59,\\ tonto, 0.59}   & \parbox{7em}{\centering\Tiny  migranti, 0.67,\\ merda, 0.66,\\ entrare, 0.66}   &  ---  & --- \\ 
%\cmidrule(lr){2-8}

\Small{christians} &  \Small{catolicos}   &   \Small{catolicos} &\parbox{7em}{\centering\Tiny falangitos, 0.61,\\ dicen, 0.59,\\ manifiesto, 0.58}  & \parbox{7em}{\centering\Tiny religiosi, 0.60, \\nazismo, 0.60,\\  cristiani, 0.60} &  \parbox{7em}{\centering\Tiny cómplice, 0.59, \\ crisis, 0.59, \\ socialmente, 0.59}  & \parbox{7em}{\centering\Tiny accadrà, 0.63,\\ summit, 0.63,\\ costi, 0.62}\\ 


\midrule

\Small{Spanish Seed Term} & \Small{English}  & \Small{Italian}  & \Small{English} & \Small{Italian} & \Small{English} & \Small{Italian} \\
%
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 %                    
\Small{negros}&\Small{blacks}&\Small{neri} & \parbox{7em}{\centering\Tiny monkey, 0.61, \\thing, 0.61,\\ today, 0.60}    & \parbox{7em}{\centering\Tiny lavoro, 0.75,\\ zingari, 0.74,\\ devono, 0.74} &  \parbox{7em}{\centering\Tiny long, 0.53, \\ case, 0.53, \\free, 0.53}
 &  \parbox{7em}{\centering\Tiny islam, 0.77,\\ parlare, 0.77,\\ islamici, 0.77} \\ 
 
\Small{gitano}&\Small{portuguese}&\Small{negro} & \parbox{7em}{\centering\Tiny beaners, 0.61,\\ chicks, 0.60,\\ young, 0.60}    & \parbox{7em}{\centering\Tiny merda, 0.66,\\ migranti, 0.65,\\
carabinieri, 0.66} &  \parbox{7em}{\centering\Tiny channel, 0.55,\\ trying, 0.55,\\ used, 0.54}
 &  \parbox{7em}{\centering\Tiny viene, 0.60,\\ cultura, 0.60,\\ basta, 0.59} \\
%\cmidrule(lr){2-8}

\Small{fachas}  & \Small{bigots} &  \Small{comunisti}   &\parbox{7em}{\centering\Tiny  muslims, 0.59,\\  muslim, 0.58,\\  fucking, 0.58}    &\parbox{7em}{\centering\Tiny migranti, 0.78,\\  immigrati, 0.78,\\  stranieri, 0.77}  &  \parbox{7em}{\centering\Tiny worse, 0.58,\\  turned, 0.57,\\ come, 0.57}  & \parbox{7em}{\centering\Tiny parla, 0.75,\\ vero, 0.74,\\ islam, 0.74}   \\ 
% \cmidrule(lr){2-7}

 %&     &    &    &  &    &     \\ 

\midrule
%
 \Small{Italian Seed Term} & \Small{English}  & \Small{Spanish}  & \Small{English} & \Small{Spanish} & \Small{English} & \Small{Spanish} \\
%
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}
 %                    
\Small{migranti} &  \Small{illegals}   &  \Small{deportarlos}  &  \parbox{7em}{\centering\Tiny fags, 0.68,\\ niggers, 0.68,\\ time, 0.68} &  \parbox{7em}{\centering\Tiny fachas, 0.78,\\ nazis, 0.78,\\ gusta, 0.78} &  \parbox{7em}{\centering\Tiny fags, 0.68,\\ niggers, 0.68,\\ time, 0.68}  & \parbox{7em}{\centering\Tiny cosas, 0.78,\\ ridículo, 0.77,\\ mejor, 0.76}  \\ 

\Small{terroristi} &  \Small{minncharges}   &  \Small{protestantes}   & \parbox{7em}{\centering\Tiny muslim, 0.66,\\ muslims, 0.65,\\ islam, 0.65}   & \parbox{7em}{\centering\Tiny nazis, 0.76,\\ fachas, 0.74, \\mejor, 0.74}  &   \parbox{7em}{\centering\Tiny yeah, 0.65,\\ around, 0.65,\\ anyone, 0.65}  &  \parbox{7em}{\centering\Tiny fascista, 0.78,\\  cosas, 0.78,\\  nazis, 0.77}   \\ 

\Small{islamici} &  \Small{islamic}   &  \Small{sionista}  &  \parbox{7em}{\centering\Tiny muslim, 0.65,\\ people, 0.65, \\real, 0.65}  & \parbox{7em}{\centering\Tiny nazis, 0.76, \\fachas, 0.76, \\nazi, 0.75}  & \parbox{7em}{\centering\Tiny around, 0.65,\\ time, 0.65,\\ anyone, 0.64}   &  \parbox{7em}{\centering\Tiny cosas, 0.79,\\ nazis, 0.78,\\ mejor, 0.78}  \\

% &     &    &    &  &    &   \\ 
\bottomrule

\end{tabular}
\end{table*}


==> DNN_Embeddings2.tex <==
\begin{table*}
\caption{Macro f-score in cross-Lingual performance of Deep Learning models using three different embeddings: mBert, Muse, and the one we built for this task CCA. These results were computed by averaging the results of five different runs of the models using five different random seeds.The numbers on bold etters represent the best performance per word-embedding type, the (*) symbol marks the best result for each training set configuration.}
\label{tab:Embeddings-DNN}
\begin{tabular}{@{}llccccccc@{}} %\toprule
		& &  &				&			&&	LSTM		& LSTM			&		\\
	Testing	& Training& Features	&FNN&	LSTM &	CNN	&	+ ATTN	&	+ CNN&	ATTN 	\\ 
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-9}

 Spanish & English  & mBert&52.94 &\textbf{54.87} &53.16 &54.05 &53.72 &53.01\\
& & Muse  &39.43 &49.78 &\textbf{51.88} &39.33 &43.02 &43.08\\
& & CCA &50.83 &50.54 &34.15 &35.89 &\textbf{56.21}* &55.21\\
%         &   & CCA	& 	&	&  & & & \\
        
%         &   & VEcMAp & 	&	&  & & & \\
% 	 	&   & with\_specificData	& 	&	&  & & & \\
%         &   & AVG & 	&	&  & & & \\
\addlinespace    

&   Italian & mBert&48.86 &58.74 &53.28 &59.06 &\textbf{59.74} &54.53\\
&&Muse&\textbf{54.53} &43.08 &43.02 &43.02 &43.02 &43.08\\
&&CCA &48.54 &51.51&51.99 &46.43 &\textbf{58.38} &44.86\\
\midrule
 Italian &   English  &mBert &51.97 &\textbf{55.85} &53.55 &48.31&51.14 &48.58\\
&&Muse &56.12 &45.28 &54.77&\textbf{57.75}* &45.22 &56.23\\
&&CCA &24.09 &\textbf{55.46 }&33.88&45.70&45.28 &52.86\\


\addlinespace    

  &  Spanish & mBert &58.51 &50.82 &60.09& \textbf{60.55} &54.01 &56.00\\
&&Muse &15.38 &\textbf{52.89} &14.60 &31.50 &45.28 &45.28\\
&&CCA &55.55 &47.10 &56.22 &\textbf{ 62.06} &50.26 &58.30\\
% 	 	&   & fineTeunedBert	& 	&	&  & & & \\
    
%         &   & CCA	& 	&	&  & & & \\
        
%         &   & VEcMAp & 	&	&  & & & \\
% 	 	&   & with\_specificData	& 	&	&  & & & \\
% 	 	&   & AVG	& 	&	&  & & & \\
\midrule
   English &  Spanish  &mBert &31.51 &37.68 &49.06 &53.27 &35.64 &\textbf{54.60 }\\
&&Muse &32.04 &30.57 &30.42 &\textbf{48.61} &35.74 &35.74\\
&&CCA &44.92 &\textbf{65.06}* &51.70 &52.44 &54.69 & 42.25\\
            % 	 	&   & fineTeunedBert	& 	&	&  & & & \\
        
%         &   & CCA	& 	&	&  & & & \\
        
%         &   & VEcMAp & 	&	&  & & & \\
% 	 	&   & with\_specificData	& 	&	&  & & & \\
% 	 	&   & AVG	& 	&	&  & & & \\
\addlinespace    

  &  Italian  &mBert &44.21 & 48.96 &42.53 & 50.09 &37.86 &\textbf{62.30 }\\

&&Muse &53.79 &46.27 &35.74 &\textbf{56.40} &35.74 & 35.74\\
&&CCA &\textbf{62.68}* &39.75 &52.75 & 44.10 &46.17 &39.12\\
% 	 	&   & fineTeunedBert	& 	&	&  & & & \\
        
%         &   & CCA	& 	&	&  & & & \\
        
%         &   & VEcMAp & 	&	&  & & & \\
% 	 	&   & with\_specificData	& 	&	&  & & & \\
% 	 	&   & AVG	& 	&	&  & & & \\
\addlinespace
\bottomrule
\end{tabular}
\end{table*}
\input{insert_crosslingual}

==> Datasets_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}\caption{Description of the datasets we used for hate speech evaluation. For each dataset  we show the number of tweets per class.}\label{tab: datasets}
\begin{tabular}{lccc}
     & \small{English} & \small{Spanish} & \small{Italian} \\
     
\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
\Small{Hateful}     & 2,920 &   1,576      & 1,291  \\ 
\Small{Non-Hateful} & 5,576 &   4,434     & 5,637   \\ 
\cmidrule(lr){1-4}
\small{Total}     & 7,496    &   6,000      & 6,928  \\        \midrule
\end{tabular}
\end{table}

==> TML_Embeddings.tex <==
\begin{table*}
\caption{Macro f-score in cross-Lingual performance Traditional Machine Learning Models using language agnostic features, LASER embeddings. These results were computed by averaging the results of five different runs of the models using five different random seeds.}
\begin{tabular}{@{}llccccccc@{}} %\toprule
		Testing& Traning  & Representation& LR & NB &	SVM	& DT			&	RF		& xgb\\
		
\cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-9}
\addlinespace

Sp\_test & En\_train & Avg(mBert)	& 49.24	&43.07	&42.97  &\textbf{ 51.79}&45.65 & 48.10\\
	 	&   & LASER	& 50.66	&30.26 & 43.00 & 48.45& \textbf{53.17*} & 49.44 \\

	 	&   & LIF	& 43.75	&41.89	&  43.04&45.58 & 43.04&\textbf{49.51 }\\
&   & Laser  + LIF	&45.54 &	41.65&43.04 &48.71&47.52& \textbf{48.36}\\        
\addlinespace    
\cmidrule(lr){2-9}
\addlinespace    

  & It\_train  &Avg(CCA) & 46.01 	&42.97	& 43.04 & 48.93& 43.94& \textbf{51.03}\\
&   &LASER	& 43.51	&48.21	&43.44  &51.17 &43.88 &\textbf{53.73}\\
	 	
 	 	&   & \textbf{LIF}	&43.05 	& 30.83 &43.04&49.73&44.99&\textbf{54.73*}\\
&   & Laser  + LIF	&43.04 &30.83& 43.04&53.55&44.54&\textbf{53.84}\\
\midrule
It\_test & En\_train  & Avg(Muse)	& 45.27	&45.27	&45.32  & \textbf{51.19}&45.32 & 47.56\\
  	 	&   & \textbf{LASER}	& 53.35	&24.86	& 45.32 &49.62 & 56.47&\textbf{53.62*} \\

	 	&   &LIF	&45.16 	&36.61	&  45.32&50.24 &46.41 &\textbf{53.49}\\
&   & Laser  + LIF	&44.95 &36.61	&45.32 &52.39&\textbf{53.20}&51.33 \\
\addlinespace    
\cmidrule(lr){2-9}
\addlinespace   
  & Sp\_train &Avg(CCA) 	& 50.25	&45.27	& 45.32 &\textbf{54.11}&45.11 &53.27\\
	              & &LASER	&47.48 	&58.15	&45.32  &52.39 & 45.32&\textbf{54.77} \\
	 	&   &LIF	&45.32 	&32.17	&45.32  & 51.58&  45.16&\textbf{51.73}\\
&   &\textbf{ Laser  + LIF}	& 45.32&22.17&45.32 &54.47&46.41&\textbf{55.98}* \\	 		 	
\midrule
En\_test & Sp\_train  &Avg(CCA)	& 36.48	&35.74	&35.74  &\textbf{51.01} &35.74 & 48.77\\

	 	&   & LASER &39.52	&49.21	&36.80  & 49.28&3817 & \textbf{51.56*
	 	}\\
	 	&   & LIF &40.97 &26.97	& 40.97 & 47.23& 40.80&\textbf{49.09}\\ &   & Laser  + LIF	& 41.59&26.97	&40.97 &40.97&40.97&49.96 \\	 	       
\addlinespace    
\cmidrule(lr){2-9}
\addlinespace  

  & It\_train  &Avg(CCA)	&\textbf{62.27}*	&36.10	&35.74 &55.06 &37.70 & 49.51\\
&   & LASER	&36.04 	&51.72	&36.39  & 49.85&36.04 &\textbf{53.22}\\

&   & LIF	& 40.97	&28.89	& 40.97 &\textbf{54.94} &42.07 &41.39 \\	 	
&   & AvgCCA  + LIF	&40.97 &50.23	&40.97 &48.82&41.59& 53.65\\	 	

\addlinespace
\bottomrule
\end{tabular}
\end{table*}

==> cross_lingual_augmentation.tex <==
\begin{table}
\centering
\caption{Classification results using data augmentation from a different language.}
\label{Table 5}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{p{24mm}|l|l|l}
\hline
Testing Set                    & Training Set                     & Accuracy & F-Score \\ \hline
\multirow{6}{*}{Spanish\_test} & Sp\_train                        &   82.43\%       &  83.42\%       \\ \cline{2-4} 
                               & Sp\_train + En\_total             & \textbf{82.91\%} & \textbf{83.78\%} \\ \cline{2-4} 
                               & Sp\_train + It\_total             & 82.69\% &  82.69\%         \\ \cline{2-4} 
                               & Sp\_train + En\_total + It\_total &82.11\%& 82.11\%        \\ \hline\hline
\multirow{6}{*}{English\_test} & En\_train                         &\textbf{80.95\%}       & 78.03\%  \\ \cline{2-4} 
                               & En\_train + Sp\_total             &80.33\%          & 76.83\%        \\ \cline{2-4} 
                               & En\_train + It\_total             &80.50\%          & 76.98\%        \\ \cline{2-4} 
                               & En\_train + Sp\_total + It\_total & 80.41\%         & \textbf{79.01\%}         \\ \hline\hline
\multirow{6}{*}{Italian\_test} & It\_train & \textbf{68.66\%} & \textbf{62.40\%} \\ \cline{2-4} 
                               & It\_train + En\_total             &67.33\%          &55.36\%         \\ \cline{2-4} 
                               & It\_train + Sp\_total             &63.33\%          &61.38\%         \\ \cline{2-4} 
                               & It\_train + En\_total + It\_total & 64.0\%         & 61.43\%      \\ \hline\hline
\multirow{6}{*}{Spanish\_manual} & Sp\_total                         &64.0\%        &63.99\%         \\ \cline{2-4} 
                               & En\_total                           &61.0\%        &60.7\%         \\ \cline{2-4} 
                               & It\_total                         &60.02\%        &55.1\%         \\ \cline{2-4} 
                               & Sp\_total + En\_total             &\textbf{66.2\% }         &\textbf{64.78\%}         \\ \cline{2-4} 
                               & En\_total + It\_total             & 62.8\%         &57.62\%         \\ \cline{2-4} 
                               & Sp\_total + En\_total + It\_total & 60.3\%          &   62.5\%       \\ \hline\hline
\end{tabular}}
\end{table}


==> hyper.tex <==
\begin{table}[h!]\caption{Hyperparameters used in the cross-lingual experiments.}
\begin{tabular}{l l l} \label{hiper}

Model & Parameters                                       &  \\ \hline
FNN   & \begin{tabular}[c]{@{}l@{}}a :\\ b:\end{tabular} &  \\ \hline
LSTM  & \begin{tabular}[c]{@{}l@{}}a:\\ v:\end{tabular}  &  \\ \hline
\end{tabular}
\end{table}

==> insert_crosslingual.tex <==
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/crosslingual_en.png}
% \caption{Testing on En\_test}
% \label{fig:westminster_lateral}
% \end{subfigure}
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/crosslingual_es.png}
% \caption{Testing on Es\_test}
% \label{fig:westminster_aerea}
% \end{subfigure}
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/crosslingual_it.png}
% \caption{Testing on It\_test}
% \label{fig:westminster_aerea}
% \end{subfigure}
% \caption{Cross Results}
% \label{fig:westminster}
% \end{figure}


==> insert_monolingual.tex <==
% \begin{figure}[h!]
% \centering
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/monolingual_en.png}
% \caption{Testing on En\_test}
% \label{fig:westminster_lateral}
% \end{subfigure}
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/monolingual_eS.png}
% \caption{Testing on Es\_test}
% \label{fig:westminster_aerea}
% \end{subfigure}
% \begin{subfigure}[b]{0.75\linewidth}
% \includegraphics[width=\linewidth]{images/monolingual_it.png}
% \caption{Testing on It\_test}
% \label{fig:westminster_aerea}
% \end{subfigure}
% \caption{Monolingual Results}
% \label{fig:westminster}
% \end{figure}


==> seed_vs_random.tex <==
\begin{table}[]\label{seed_vs_random}
\caption{For each language, 10 thousands tweets were recovered by using the discovered terms and 10 thousands randomly. This table shows the percentage of the tweets that are hateful in each of this  groups of tweets}
\begin{tabular}{c c c c c c}

\multicolumn{2}{c}{English} & \multicolumn{2}{c}{Spanish} & \multicolumn{2}{c}{Italian} \\ 
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
Random& Queried &Random& Queried &Random& Queried\\ 
 & & & &  & \\ 
\end{tabular}
\end{table}
